An optimization approach to locally-biased graph algorithms

Locally-biased graph algorithms are algorithms that attempt to find local or small-scale structure in a large data graph. In some cases, this can be accomplished by adding some sort of locality constraint and calling a traditional graph algorithm; but more interesting are locally-biased graph algorithms that compute answers by running a procedure that does not even look at most of the input graph. This corresponds more closely to what practitioners from various data science domains do, but it does not correspond well with the way that algorithmic and statistical theory is typically formulated. Recent work from several research communities has focused on developing locally-biased graph algorithms that come with strong complementary algorithmic and statistical theory and that are useful in practice in downstream data science applications. We provide a review and overview of this work, highlighting commonalities between seemingly-different approaches, and highlighting promising directions for future work.

==> sec-cut-text.tex <==
\section{Text that has been cut}


\section{Intro}

Motivated by these very large-scale data analysis applications where only small meaningful clusters exist and where the graphs are so large that iterating over all edges and nodes is measured in minutes or hours, recent work has focused on \emph{locally-biased graph algorithms}.
This refers to a broad class of algorithms that are designed to take as input a large graph, e.g., a billion node social or information network, and to solve problems that are in some sense ``nearby'' an exogenously-specified ``seed set'' of nodes.
While these algorithms are often very useful in practice, and while many of them have connections with heuristic procedures that practitioners often apply to their data, a distinguishing feature of them is their non-trivial algorithmic and/or statistical theory.


%The types of results differ, but there are strong relationships between the methods. 

%More generally, our focus on clustering so far is that the problem of finding good partitions or clusters is ubiquitous, and most of the local graph methods have explicit or implicit connections with local versions of finding good clusters.
%We should emphasize, however, that the basic properties that are used to find good clusters are also useful for other problems.
%For example, the isoperimetric properties underlying Cheeger's inequality that is the reason that the usual unsupervised global spectral clustering algorithms lead to good clusters is useful in other ways: to get good classification in supervised settings; and to get classification/regression results in the semi-supervised/transductive setting.
%\textcolor{red}{XXX.  MM TO GO INTO MORE DETAILS ON THIS.}
%\begin{itemize}
%\item
%The dual of MOV gives the embedding into a locally-biased complete graph, and so it can be viewed as doing a local prior.
%\item
%Toke formulated the problem as semi-supervised eigenvectors.
%\item
%LE is used for all sorts of things in ML, and these provide a locally-biased version of those.
%\item
%More generally, something.
%\end{itemize}
%Relatedly, if we can split a graph into two pieces that don't talk with each other, then we can do things like recursive partitioning, divide and conquer, control statistical inference, etc.
%Thus, although most of what we will discuss here has to do with the the unsupervised clustering problem, one can expect that many of these results can be extended to local and locally-biased versions of supervised, semi-supervised, and transductive settings.
%
%
%Spectral versus flow.
%Many of the algorithms involve some sort of diffusion (\textcolor{red}{random walk}) and so have a natural interpretation in terms of spectral approximation algorithms, while other algorithms, sometimes for quite different problems, are flow-based algorithms, either explicitly or implicitly (\textcolor{red}{not sure what explicitly or implicitly means here}).

%Finally, we'll present a novel analysis of a particularly widely-used spectral based method. 


%\section{Some references}
%\textfinish{David---I don't think we need this section, it should be integrated into the text.}
%
%Here are some relevant papers from MM.
%I probably am missing some, which I will think of when I give it more thought as we iterate.
%Also, it is certainly in need of more from KF and/or DG.
%\begin{itemize}
%\item
%\cite{Spielman:2004} (or a related paper) is where they first described their algorithm for local graph partitioning using local random walks that uses ideas from.
%\cite{andersen06local} is the ACL paper that improves on ST.
%\cite{Chung07_heatkernelPNAS} is a local spectral method that uses heat kernels.
%\cite{AP09} is the Andersen-Peres evolving set method.
%\item
%\cite{chung07_fourproofs} is probably worth citing, although it provides an odd taxonomy.
%\cite{Chung07_localcutsLAA} is probably also worth citing.
%\item
%\cite{Chung:1997}: The basic spectral graph theory book to cite.
%\item
%\cite{andersen08soda} is the AL paper that does flow-improve that improves MQI.
%\cite{kevin04mqi} is the MQI paper.
%\cite{Gallo:1989} is (I think---check) the GGR paper that is prior art for the MQI paper.
%(We need to be careful about the differences between single and multi-commodity flow methods.)
%\item
%\cite{LLDM08_communities_CONF,LLDM09_communities_IM,LLM10_communities_CONF} is the LLDM empirical evaluation.
%\cite{Jeub15} is the Jeub extension.
%\item
%\cite{andersen06seed}: This paper used a local spectral method (the ST method I think) to look at communities.
%\item
%\cite{MO11-implementing} is the Orecchia implicit regularization of early-stopped diffusions.
%\cite{PM11} is the statistical interpretation of the Orecchia implicit regularization result.
%\cite{GM14_ICML} is the Gleich implicit regularization for ACL.
%\cite{GM15_KDD} is the Gleich robustification paper.
%\item
%\cite{ZLM13} is the local algorithm for finding well-connected clusters.
%\item
%\cite{MOV12_JMLR} is the MOV local spectral paper.
%\item
%\cite{spielman96_spectral,spielman07_spectral}: This is the paper that shows that spectral partitioning works where it is usually applied. 
%(It also has a nice historical review.)
%\cite{guatterymiller98}: This is the paper that shows that spectral partitioning doesn't work on cockroaches, etc.
%\item
%\cite{Leighton:1988,Leighton:1999} is the LR result, with the $\log n$, etc.
%\cite{LLR94_CONF} is the LLR paper that talks about embeddings of flow, etc.
%\cite{HLW06_expanders} is the HLW review (which also describes the embeddings nicely).
%\item
%\cite{Arora:2004,ARV_CACM08} is the ARV method.  
%(There are a bunch of other optimization-based variants we'll need to cite.)
%\cite{LMO09} is the only empirical evaluation of ARV-type methods.
%\item
%\cite{OZ14} is the Orecchia-Zhu paper on a local flow improve method.
%\cite{Din06} is Dinic's algorithm, which is used by Orecchiz-Zhu to search blocking flows in a particular order to stay local in a manner somewhat like how diffusions spread out.
%\item
%There are lots of other ``hueristic'' methods for global graph partitioning that we won't discuss but whose ideas can sometimes be grafted onto these local methods.
%\cite{Kernighan:1970,FM82} are local search methods.
%\cite{karypis98_metis,karypis98metis} is the multilevel METIS method.
%\end{itemize}




%We shall illustrate and explain locally-biased graph procedures that can identify both of the sets in Figure~\ref{fig:small-cluster} within seconds---albeit without proof of optimality. 
In this overview paper, we will cover recent work of global and local graph algorithms, touching on each of these topics, reviewing complementary aspects, and focusing on optimization questions.
We split this paper into three parts, optimization objectives, global and local algorithms. 
%Our motivation for these methods is that they are very useful in characterizing the large-scale and small-scale properties of real data graphs.
First we will present optimization objectives which by consensus quantify the notion of a cluster in a graph. The optimization problems that we present are NP-hard, thus cannot be optimized in polynomial time.   
Then we discuss state-of-the-art polynomial time relaxations that result in spectral or max-flow problems. Second, we present an overview of locally-biased graph partitioning methods in terms of \emph{flow-based methods} and \emph{spectral-based methods}. 
Finally, we illustrate their performance in practice and comment on the implicit or explicit regularization that is applied by each algorithm. 


\section{Regularization, Beyond $\ell_1$ and $\ell_2$}


It is easy to see that the above problem is a continuous representation of $s$-$t$ Min-Cut problem.
The constraints $x_s=1$ and $x_t=0$ represent regularization such that the trivial solution of a constant
vector $x$ is obtained. At the same time these two constraints affect the separation of the graph in two parts
such that the nodes $v_s$ and $v_t$ are in different parts of the partition.

The approximation is based on the distortion error of embedding the semi-metric to
the so called $\ell_1$-metrics set, see \cite{} (\textcolor{red}{Leighton Rao}) for details.

\paragraph{Theoretical issues: combining spectral and flow.}
\textcolor{red}{The material below is also covered in the SDP section, we need to combine them.}


Although it isn't our main focus, we comment briefly on one set of well-known results and how it fits in with our discussion.
A natural question in the above is whether one can combine the complementary ideas from spectral and flow to obtain improved results.
The answer is yes, and this is the ARV algorithm.
It (1) can be written as a tighter relaxation of the expansion/conductance problem, (2) can be written as an SDP, (3) provides improvement over spectral as well as LR, (4) leads to related optimization-based methods/approaches such as KRF and MWUM that lead to similar improvements.
XXX.  GIVE THE OBJECTIVE AND RELAXATION AND RESULTS AND LEAVE IT AT THAT.
BTW, also, LMO showed that the practice follows the theory for graphs up to thousands to tens of thousands of nodes~\cite{LMO09}, but, aside from this, these methods haven't really been implemented.
XXX.  WE'LL PROBABLY SAY IN THE CONCLUSION THAT LOCAL ARV METHODS ARE OPEN.

\subsection{Embedding aspects}\label{subsection:embeddings}
\textcolor{red}{I have to embed ( :-) ) this section in previous sections since most of the material below is already mentioned above.}


These two approaches have an interpretation in terms of embeddings (which is of theoretical interest, but which also can be seen empirically), and this provides a way to think of the two together as complementary (in the global case, but we will do the local case below).

To start, return to min-cut, and note that that objective, while tractable, often leads to trivial solutions, in that it cuts on a very small number of nodes, e.g., one or two.
Thus, it is common to normalize by the volume.
(Alternatively, one could have a balance constraint or use methods that explicitly or implicitly provide a bias toward large sets of nodes.)
In this case, one can define the expansion of a set of nodes to be the usual expansion-SA-to-Volume measure.
XXX.  DEFINE.
If the graph is weighted or has variable degrees, then one could define the conductance to be the usual conductance-SA-to-Vol measure.
(They are the same for unweighted/degree-regular graphs, but not otherwise and the differences are important in theory/practice.)  
Note that the input to these objectives is just a graph $G=(V,E,W)$.

These objectives are intractable, but they capture the qualitative idea of what most people think of by clusters---relatively large, relatively a lot of stuff inside, relatively less interaction between the cluster and its complement.
The point is that spectral and flow both give approximation algorithms for expansion/conductance.
Spectral relaxes one way, i.e., the $\{-1,1\}$ constraint to being $\pm1$ on average, and this can be solved by computing eigenvectors or diffusions
Flow relaxes another way, i.e, the $\{0,1\}$ constraint to be a metric, and this can be written as the solution of an LP, which can then be solved with flow methods like Dinic or related methods.

From this embedding perspective, it is clear that spectral embeds the graph not just on a like, and it then does a sweep cut, but it also embeds the graph in a complete graph, i.e., the Laplacian of a complete graph, and it is here that the duality is the tightest.
It is here that the quadratic approximation result of Cheeger arises.
And note that for spectral methods random walks mix quickly on constant-degree expanders and slowly on line graphs, and this can be sued to construct the Guattery-Miller cockroach graphs.
XXX.  SOMETHING ABOUT CONNECTIONS WITH L2.
Similarly, flow methods embed you in an $\ell_1$ space, and Bourgain's embedding lemma says that an $O(\log n)$ distortion can be expected, and this happens on constant degree expanders.

We have gone through this in some detail since many of the ideas are essential for constructing local versions of these methods.
Many of these results are ``obvious'' to certain research areas and not even thought about by other research areas, so we went through them in the more well-developed global partitioning area, so we can draw similarities with local methods.

\subsection{Some additional observations}

There is, of course, the usual theory-practice gap.
Theoretical work typically considers the problem of two clusters, and applied work is often more interested in more than two clusters.
The latter, while also using a lot of algorithm engineering, often uses ideas that boil down to the former.
Here, we mention a few things.

\paragraph{Practical issues: going beyond spectral and flow.}

Global graph partitioning methods basically boil down to some combination of spectral and flow, also couples with ideas like multi-resolution.
The canonical example of this is METIS~\cite{karypis98_metis,karypis98metis}.
This, coupled with doing things ``right,'' e.g., doing the sweep cut right with spectral of doing something analogous like Goldberg does with flow algorithms, can have a big effect on the quality of the result.
We won't go into a lot of detail about this, but we expect that a lot of these ideas can also lead to improved local and


\section{Spectral methods}

%A second way starts with the idea that we can compute eigenvectors of matrices associated with graphs.  
%For example, for a regular graph compute the top eigenvector of an adjacency matrix, or equivalently the bottom eigenvector of the Laplacian, and for a non-regular graph compute the bottom eigenvector of the normalized Laplacian.
%If we do that, then we can use Cheeger's inequality and get quadratically-good approximation bounds.
%This shows that any eigenvector with Rayleigh quotient leads to similar results.
%Alternatively, since the bottom nontrivial eigenvector of the normalized Laplacian is the limit state of random walks, we can run random walks to the asymptotic or pre-asymptotic state, and we can get similar results.
%The interpretation is the slowest mixing direction of the random walk.
%This shows that these spectral methods don't compute cuts but instead try to find bottleneck to mixing.
The material in this section is based on \cite{S11}. 
Then 
$$
vol(E(S,S^c)) = \frac{x^T L x}{(c_1-c_2)^2} %= \frac{\sum_{i=1}^{|\V|}\sum_{j=1}^{|\V|} A_{ij}(x_i - x_j)}{(c_1-c_2)^2}
$$
and
$$
x^TDx = c_1^2 vol(S) + c_2^2 vol(S^c). %= vol(S)vol(S^c)\left(\frac{c_1^2}{vol(S^c)} + \frac{c_2^2}{vol(S)}\right).
$$
Depending on how we define $c_1$ and $c_2$ we obtain different problems. For example, if 
$$
c_1= \sqrt{\frac{vol(S^c)}{vol(S)}}, \ c_2= -\sqrt{\frac{vol(S)}{vol(S^c)}}
$$
then the following problem
\begin{align}\label{spcutLD}
\mbox{minimize}   & \quad \frac{x^TLx}{x^TDx} \\\nonumber
\mbox{subject to} &\quad x\in\{c_1,c_2\}^{|\V|}
\end{align}
is equivalent to the Sparsest-Cut problem \eqref{spcut}.
If $c_1=1$ and $c_2=0$ then \eqref{spcutLD} is equivalent to the Minimum-Isoperimetry problem \eqref{isop}. It is clear that for different values of $c_1$ and $c_2$ we impose different 
regularization on the optimal partition of the graph. However for any values of $c_1$ and $c_2$ problem \eqref{spcutLD} is still NP-hard.
A possible way to overcome this difficulty is to relax the solution set to $\{u\in\mathbb{R}^{|\V|} \ | 1_{|\V|}^T D u = 0\}$, where $1_{|\V|}$ is a column vector of ones of length $|\V|$.
This relaxation is equivalent to finding the second largest eigenvalue of the normalized graph Laplacian $\mathcal{L}$, which justifies the name spectral relaxation.
The relaxed problem is 
\begin{align}\label{spcutLD}
\mbox{minimize}   & \quad \frac{x^TLx}{x^TDx} \\\nonumber
\mbox{subject to} &\quad x\in\{u\in\mathbb{R}^{|\V|} \ | \ 1_{|\V|}^T D u = 0\},
\end{align}
which is a non-convex problem, but all local solutions are of the same importance since all have the same objective value.
The local solutions differ only by a positive constant factor and a sign change. The reason for imposing the orthogonality constraint $1_{|\V|}^T D x = 0$
is because otherwise \eqref{spcutLD} has a trivial solution, the eigevector $D^{1/2} 1_{|\V|}$ (any other constant vector can be used instead of $1_{|\V|}$)
of the zero (the smallest) eigevalue of $\mathcal{L}$. 

Let us define $\delta_S(v_i,v_j) = |x_i - x_j|^2$.\ Using $\delta_S$ we can rewrite the numerator in the objective function as
$$
x^T L x = \sum_{i=1}^{|\V|}\sum_{j=1}^{|\V|} C_{ij}\delta_S(v_i,v_j).
$$
Another way of viewing the spectral relaxation is by noticing that if instead of defining $x : \V \to \{c_1,c_2\}$ to be an indicator function, we allow it to be any
arbitrary function $x: \V \to \mathbb{R}$, then we relax the cut-metric $\delta_S$ to be the Euclidean square distance. 
%Using this point-of-view of the spectral relaxation 
%the reader should be able to see how the diagram in Figure \ref{subsubsec:spcut} is obtained. 



\section{Local methods}

\subsection{The Local-Isoperimetry Problem}

Recall that we introduced the Sparsest-Cut and Minimum-Isoperimetry problems as regularizations of the Min-Cut problem that were designed to achieve some control over the size of the set identified. The Local-Isoperimetry problem is an integer problem that adds more regularization (or a constraint) to achieve a local solution~\cite{MOV12_JMLR}. The problem depends on a graph $G$ and a reference set $R$ that must be contained within the solution. We also make the size of the final set a parameter $k$. The new program is 
\begin{align}
\hat{\phi}(\G;R,k) \quad := \quad 
\mbox{minimize}   & \;   \tilde{\phi}(S)= \frac{vol(E(S,S^c))}{vol(S)} \\\nonumber
\mbox{subject to} & \;  S\subset \V,\ vol(S) \le k \\ \label{eq:localiso}
& \; R \subseteq S. \nonumber
\end{align}
It differs from the Minimum-Isoperimetry problem because we have replaced the volume bound with a constant $k$ and require that the solution set $S$ contain the reference set $R$. The idea with this problem is that we wish to localize the solution to the Minimum-Isoperimetry problem around a subset of nodes $R$. We'll often take $R$ to be a single node. 

Note that if $k = vol(G)$ then this problem may be solved as a parametric flow problem using techniques akin to those in~\cite{HochbaumNcutprime}. If $k = vol(G)/2$, then we are able to use $|V|$ runs of this algorithm to solve the Minimum-Isoperimetry problem by setting $R$ to be each vertex. So solving this is NP-hard in general.

We illustrate one counter-intuitive feature of this problem in Figure~\ref{fig:local-iso}. First, let us note that one of the global solutions of the Minimum-Isoperimetry problem must be a connected subgraph. However, the solution set of the Local-Isoperimetry problem may be a disconnected graph. This occurs if there is another set in the graph with a sufficiently small isoperimetry value such that it is better to pay the price for disconnecting the reference graph $R$ and returning the union of the two. 

\begin{figure}[t]
	\subfigure[The Local-Isometry solution may be disconnected. The singleton node is the set $R$.]{\includegraphics[scale=0.33]{U3A-local-iso-1-500}}\hspace{0.01\linewidth}%
	\subfigure[Increasing $k$ results in a connected set for this problem.]{\includegraphics[scale=0.33]{U3A-local-iso-1-5000}}
	\caption{The singleton node in (a) is not a bug. The single disconnected node was the set $R$.  \textfinish{Add more discussion.} \textfinish{add PGP figures}}
	\label{fig:local-iso}
\end{figure}	


==> sec-l2-l1.tex <==
\section{Regularization, $\ell_2$ versus $\ell_1$}

In the previous section we followed a theoretical computer science perspective. We discussed tractable combinatorial problems, i.e.,
min-cut and $s$-$t$ min-cut, and NP-hard combinatorial problems, i.e., minimum conductance and isoperimetry. 
We discussed how to relax the latter NP-hard problems in order to obtain continuous versions that are ``good" approximations in terms of worst-case objective value. 

In this section we make a step back and study the regularization properties that are imposed by min-cut and certain spectral problems. 
Understanding the regularization properties that are imposed by each problem on the solution will allow us to understand the structure
of the output solution in practice. In subsequent sections we will use the regularization problems by min-cut and spectral to understand 
what properties are imposed on the solution by current state-of-the-art local algorithms.  

\paragraph{Properties of $s$-$t$ Min-Cut} We now discuss regularization properties for the $s$-$t$ min-cut problem.
Similar properties hold for min-cut since this is the best $s$-$t$ min-cut over all pairs of nodes in $\V$.
It can be shown \cite{} that the following optimization problem
\begin{align}\label{eq:mincutL1}
\nonumber
\mbox{minimize}             & \quad  \|Bx\|_{1,C}\\
	  \mbox{subject to} & \quad x_s =1, \ x_t = 0 \\\nonumber
	  			      &\quad x\ge 0.
\end{align}
is equivalent to $s$-$t$ min-cut, which we introduced in Section \ref{subsec:mincutmaxflow}.
The solution to $s$-$t$ min-cut is binary and lies in $[0,1]^{|\V|}$, see \cite{}. Thus, the solution 
defines a partition $S, S^c$.
%Obviously the solution to this problem is any constant vector, i.e., all components of $x$ have the same value.
%We can avoid this issue by adding two constraints
%\begin{align}
%\nonumber
%\mbox{minimize}             & \quad  \frac{|\V|}{2}\|Bx\|_{1,C}\\
%	  \mbox{subject to} & \quad \|x\|_1 = 1, \\\nonumber
%	  			      & \quad x^T 1_{|\V|}=0.
%\end{align}
%The first constraint is to avoid the all zeros solution and the second constraint is to avoid constant solutions.
%This problem is equivalent to the Min-Cut problem 
%which was introduced in Subsection \ref{subsec:mincutmaxflow}. The solution to \eqref{eq:mincutL1} lies in $[-1/|\V|,1/|\V|]^{|\V|}$, i.e., its a binary solution.
%The constant in the right-hand-side of the first constraint is chosen arbitrarily, it can be replaced with any constant and the solution
%will still lie in $[-\alpha,\alpha]^{|\V|}$ for some positive constant $\alpha$. Furthermore, we can replace the constraint 
%$x^T 1_{|\V|}=0$ with other constraints depending on our aim and still obtain binary solutions. In fact, any affine constraint that defines
%a feasibility set that is perpendicular to the constant vector if combined with an $\ell_1$ norm in the objective and $\ell_1$ norm length constraint, 
%then this is sufficient to result in an optimization problem with a binary solution. The constraint $x^T 1_{|\V|}=0$ is only responsible for the uniqueness 
%of the solution. (\textcolor{red}{It might be better to prove this, or provide a figure?}).
%For example the $s$-$t$ Min-Cut problem which replaces the linear constraint $x^T 1_{|\V|} = 0$ with the linear constraints $x_s = 1$ and $x_t = 0$,
%where $s$ is the source and $t$ is the sink nodes. The optimal solution of $s$-$t$ Min-Cut is also binary, i.e., lies in $[0,1]^{|\V|}$.
%It is the combination of two properties, i.e., the $\ell_1$ norm in the objective and the $\ell_1$ norm in the length constraint
%that are responsible for obtaining a binary solution. If any of these is not used then the solution is not guaranteed to be binary. 
Since we assumed that the given graph has edges with unit-weights then the $s$-$t$ min-cut objective penalizes partitions $S,S^c$ that have 
many outgoing edges from $S$ to $S^c$. Intuitively, this implies that min-cut looks for partitions which have clear boundaries. 
For many applications, depending on the given graph such a property might be very important. Later on we will see that there are local
algorithms which preserve this property close to a given input seed set. 
%Notice that one could replace only the $\ell_1$ norm in the objective of \eqref{eq:mincutL1} with the $\ell_2$ norm and 
%the solution of the resulting problem can be ``smooth" instead of binary. It is clear that the $\ell_1$ norm in the objective
%is necessary to obtain a solution 

\paragraph{Properties of spectral} Let us now replace the $\ell_1$ norm in \eqref{eq:mincutL1} with the $\ell_2$ norm to obtain the following problem
\begin{align}\label{eq:spectralL2}
\nonumber
\mbox{minimize}             & \quad  \|Bx\|_{2,C}\\
	  \mbox{subject to} & \quad x_s =1, \ x_t = 0 \\\nonumber
	  			      &\quad x\ge 0.
\end{align}
From the preliminaries we know that $\|Bx\|_{2,C} = x^T L x$. This problem is related to spectral relaxation \eqref{spcutLD}.
The only difference between \eqref{eq:spectralL2} and \eqref{spcutLD} is that we do not scale the $\ell_2$ norm in the constraint 
with the diagonal matrix $D$. This means that we do not put weights on nodes based on their degree, i.e., all nodes are of the same 
importance. Similarly to our discussion on spectral relaxation it can be shown that problem \eqref{eq:spectralL2} is a relaxation of the Minimum-Conductance and Minimum-Isoperimetry problems where
all nodes are of the same importance. However, in this section our focus is the properties imposed by the $\ell_2$ norm and not the relaxation properties of problem \eqref{eq:spectralL2}.
The solution to \eqref{eq:spectralL2} satisfies 
$$
L x = \lambda_2 x,
$$
where $\lambda_2$ is the second smallest eigenvalue of $L$ for a unit-length eigenvector $x$. Since $L$ is the Laplacian operator of the given graph,
then the eigenvector which satisfies the previous equation can be seen as the solution to a diffusion process. 
This means that the solution to problem \eqref{eq:spectralL2} is generally ``smooth", meaning that
the values of the components of $x$ are in $\mathbb{R}$ and they are not binary. This is an important difference between \eqref{eq:mincutL1} and \eqref{eq:spectralL2},
which is due to the geometry that $\ell_1$ and $\ell_2$ norms define. Intuitively, the ``smoothness" of the solution given by spectral relaxation implies that
we loose the property of \eqref{eq:mincutL1}, which is to preserve boundaries. If one takes a clustering perspective, then this drawback can be fixed by combining spectral with some sweep procedure which will possibly 
ignore components of $x$ with very small values, i.e., nodes outside the boundary. This two step-procedure is provably at most as good as \eqref{eq:mincutL1} if our objective is to find the best partition with the fewest outgoing edges. 
However, one should not conclude that using $\ell_1$ norm than $\ell_2$ defines a better geometry. The decision between $\ell_1$ and $\ell_2$ is application depended. If one wants to preserve boundaries then they should use the $\ell_1$ 
norm. If one wants to perform a diffusion on a given graph, then one should use the $\ell_2$ norm.


==> sec-outline.tex <==

Outline:

Intro -- I think it's good

Continue -- the problem of minimizing conductance

Skip the long background (don't have room); shrink to a few paragraphs
 * Focus on conductance (or should we call it isoperimetry)
 * Focus on spectral relaxations vs. metric relaxations/multicommodity flow
 * Focus on Cheeger inequality
 
Localizing with the augmented graph

  Intuition
  MQI - exactly solve conductance within a set of nodes
  FlowImprove - weaken the restrictions
  LocalFlowImprove - make it strongly local
  SpectralMQI (Fan Chung) - spectral within a given set of nodes
  MOV - spectral akin to MOV 
  ACL / l1-ACL - add l1 to make it local
  
A new convergence result for ? 

Perspectives on local graph clustering (moved from intro)
Open problems
